A logician's view of graph polynomials

Graph polynomials are graph parameters invariant under graph isomorphisms which take values in a polynomial ring with a fixed finite number of indeterminates. We study graph polynomials from a model theoretic point of view. In this paper we distinguish between the graph theoretic (semantic) and the algebraic (syntactic) meaning of graph polynomials. We discuss how to represent and compare graph polynomials by their distinctive power. We introduce the class of graph polynomials definable using Second Order Logic which comprises virtually all examples of graph polynomials with a fixed finite set of indeterminates. Finally we show that the location of zeros and stability of graph polynomials is not a semantic property. The paper emphasizes a model theoretic view and gives a unified exposition of classical results in algebraic combinatorics together with new and some of our previously obtained results scattered in the graph theoretic literature.

==> MRK-uzeros.tex <==
\section{The location of zeros of univariate graph polynomials}
In \cite{ar:MakowskyRavveBlanchard2014}
we showed that the location of zeros of a univariate graph polynomial $P(G;X)$
may vary dramatically if we replace  $P(G;X)$ by a d.p.-equivalent (s.d.p.-equivalent ) 
graph polynomial $Q(G;X)$.
In fact, 
in \cite{ar:MakowskyRavveBlanchard2014}
we stated without detailed proof  
that if $P(G;X)$ is $\SOL$-definable, so is $Q(G;X)$. 
In this section we not only make this statement precise, but also
discuss how this affects our special graph polynomials such as generating functions of induced (spanning)
subgraphs or Harary and generalized chromatic polynomials.

\subsection{Making the polynomial basis explicit}

Let $\Gamma = \{ g_i(X): i \in \N \}$ be a family of polynomials $g_i(X) \in \Z[X]$
where each $g_i(X)$ is of degree $i$.

Typical examples of $\Gamma$ are given by 
$g_i(X)=X^i$, 
$g_i(X)=(-X)^i$, 
$g_i(X)={X \choose i}$, 
$g_i(X)= X_{(i)} =(X)\cdot(X-1)\cdot \ldots \cdot (X-i+1)}$.
In the case of the defect (acyclic) matching polynomial
we have $g_i(X) = (\frac{-1}{X^2})^i$.

Let $\Gamma$ be as above, and let $\cC$ ($\cD$) be a graph property 
(closed under under addition and removal of isoltaed vertices). We define:

\begin{enumerate}[(i)]
\item
$P_{\cC, \Gamma}^{ind}(G;X)=
\sum_{A \subseteq V(G)} g_{|A|}(X)$.
\item
$P_{\cD, \Gamma}^{span}(G;X)=
\sum_{F \subseteq E(G)} g_{|F|}(X)$
\item
Let
$\chi_{\cC}(G;X) = \sum_i c_i(G) X^i$.
Then
$\chi_{\cC, \Gamma} = \sum_i c_i(G) g_i(X)$.
\item
More generally, for any graph polynomial $Q(G;X) = \sum_i q_i(G) X^i$
we put $Q_{\Gamma}(G;X)= \sum_i  q_i(G) g_i(X)$.
\end{enumerate}






